Escaping Saddle Points for Zeroth-order Nonconvex Optimization using Estimated Gradient Descent

Gradient descent and its variants are widely used in machine learning. However, oracle access of gradient may not be available in many applications, limiting the direct use of gradient descent. This paper proposes a method of estimating gradient to perform gradient descent, that converges to a stationary point for general non-convex optimization problems. Beyond the first-order stationary properties, the second-order stationary properties are important in machine learning applications to achieve better performance. We show that the proposed model-free non-convex optimization algorithm returns an $\epsilon$-second-order stationary point with $\widetilde{O}(\frac{d^{2+\frac{\theta}{2}}}{\epsilon^{8+\theta}})$ queries of the function for any arbitrary $\theta>0$.

==> lem1proof.tex <==
\subsection{Proof of Lemma \ref{lemma_GE}}\label{prooflem1}

\begin{proof}
For a function $f$ satisfying $l$-smooth, we define Gaussian smooth function $f_v(\bm{x})=\mathbf{E}_{\bm{u}}[f(\bm{x}+v\bm{u})]$, where $\bm{u}$ is a $d$ dimensional standard Gaussian random vector $\bm{u}\sim\mathcal{N}(0,\mathbf{I}_d)$ and $v\in(0,\infty)$ is smooth parameter. \citep{nesterov2017random} Eq. 21 in section 2 shows that
\begin{equation}
\nabla f_v(x)=\mathbf{E}_{\bm{u}}[\frac{f(\bm{x}+v\bm{u})-f(\bm{x})}{v}\bm{u}]
\end{equation}
We define a gradient estimator $\hat{\nabla}=\frac{1}{m}\sum_{i=1}^{m}\frac{f(\bm{x}+v\bm{u})-f(\bm{x})}{v}\bm{u}$ so that $\mathbf{E}[\hat{\nabla}]=\nabla f_v(\bm{x})$.
From \citep{nesterov2017random} Lemma 3 and Theorem 4, we know that for any function $f$ satisfying $l$-smooth (Notice in the proof of the first inequality in Theorem 4, no convexity is needed) and any $\bm{x}\in\mathbb{R}^d$, the following are always true:
\begin{equation}\label{fv_bound}
\Vert\nabla f_v(\bm{x})-\nabla f(\bm{x})\Vert\leq\frac{v}{2}l(d+3)^{\frac{3}{2}}
\end{equation}
\begin{equation}\label{var_bound}
\frac{1}{v^2}\mathbf{E}_{\bm{u}}[\{f(\bm{x}+v\bm{u})-f(\bm{x})\}^2\Vert\bm{u}\Vert^2]\leq\frac{v^2}{2}l^2(d+6)^{3}+2(d+4)\Vert\nabla f(\bm{x})\Vert^2
\end{equation}
To give the distance between $\hat{\nabla}$ and $\nabla f$ is less than $\hat{\epsilon}$, we split the difference to two terms. Here we only consider $0<\hat{\epsilon}<1$.
\begin{equation*}
\Vert\hat{\nabla}-\nabla f\Vert\leq\Vert\nabla f_v-\nabla f\Vert+\Vert\hat{\nabla}-\nabla f_v\Vert
\end{equation*}
Choosing $v=\frac{\hat{\epsilon}}{c'l(d+3)^\frac{3}{2}}$, where $c'>1$ is a constant will be defined later, we have $\Vert\nabla f_v-\nabla f\Vert\leq\frac{\hat{\epsilon}}{2}$ based on Eq. \eqref{fv_bound}. To bound the second term, noticing that $\mathbf{E}[\hat{\nabla}]=\nabla f_v(\bm{x})$, choose $\bm{s}_i=\frac{f(\bm{x}+v\bm{u})-f(\bm{x})}{v}\bm{u}-\nabla f_v$ and $\bm{s}_i^{'}=\bm{s}_i+\nabla f_v$. We immediately know $\mathbf{E}[\bm{s}_i]=0$, and the variance of $\bm{s}_i$ can be bounded by
\begin{equation*}
\begin{aligned}
\mathbf{E}[\Vert\bm{s}_i\Vert^2
]&=\Vert\bm{s}_i^{'}-\nabla f_v\Vert^2
\overset{(a)}\leq \mathbf{E}[\Vert\bm{s}_i^{'}\Vert^2]+B\\		
&\overset{(b)}\leq 2(d+5)B^2+\frac{v^2l^2}{2}(d+6)^3\\
&\overset{(c)}\leq 2(d+5)B^2+\frac{4\hat{\epsilon}^2}{c'^2}\\
&\overset{(d)}\leq 2c'^2(d+5)B^2 =: \sigma^2
\end{aligned}
\end{equation*}
where step $(a)$ follows from $\mathbf{E}[\bm{s}_i^{i}]=\nabla f_v$ and $\Vert\nabla f\Vert\leq B$ in the assumption. By choosing $B>1$ and using Eq. \eqref{var_bound}, step $(b)$ is straight forward. Step $(c)$ holds due to the definition of $v$. Step $(d)$ follows that we omit the term with $\hat{\epsilon}^2$ by multiplying $c'^2>4$ to the first term.\\
By $l$-smooth, we have
\begin{equation*}
\begin{aligned}
\Vert f(\bm{x}+v\bm{u})-f(\bm{x})\Vert\leq vB\Vert \bm{u}\Vert+\frac{lv^2}{2}\Vert\bm{u}\Vert^2
\end{aligned}
\end{equation*}
Thus, the norm of $\bm{s}_i$ can be bounded as:
\begin{equation}\label{si_bound}
\begin{aligned}
\Vert\bm{s}_i\Vert\leq\frac{\Vert f(\bm{x}+v\bm{u})-f(\bm{x})\Vert\Vert\bm{u}\Vert}{v}+B
\leq B+B\Vert \bm{u}\Vert^2+\frac{lv}{2}\Vert\bm{u}\Vert^3
\end{aligned}
\end{equation}
However, $\bm{u}$ is a Gaussian random vector, we can't bound it directly. But we can say, given some constant $a\geq 0$, 
\begin{equation}\label{p_bound}
	P(\Vert\bm{u}\Vert>a)\leq p
\end{equation} 
where $p$ is some probability we will calculate in followings.

Assume $\bm{u}\sim\mathcal{N}(0,\mathbf{I}_d)$, \citep{nesterov2017random} Lemma 1 tells us $E\Vert\bm{u}\Vert^2\leq(d+2)$. Consider random variable $e^{t\Vert\bm{u}^2\Vert}$, where $t$ is a constant. We immediately know $e^{t\Vert\bm{u}^2\Vert}$ is non-negative and $E[e^{t\Vert\bm{u}^2\Vert}]=e^{tE[\Vert\bm{u}^2\Vert]}<\infty$. Thus, by using Markov's inequality, for $t>0$, we have:
\begin{equation}\label{norm_bound}
\begin{aligned}
P(\Vert\bm{u}\Vert^2>a^2)&=P(e^{t\Vert\bm{u}^2\Vert}>e^{ta^2})\leq\frac{E[e^{t\Vert\bm{u}^2\Vert}]}{e^{ta^2}}\\
&=\frac{E[e^{t(u_1^2+u_2^2+...+u_d^2)}]}{e^{ta^2}}=\frac{\prod_{i=1}^{d}E[e^{tu_i^2}]}{e^{ta^2}}\\
\end{aligned}
\end{equation}
Because the co-variance matrix is Identity, thus $u_1,u_2,...,u_d$ is i.i.d and $u_i\sim\mathcal{N}(0,1)$
\begin{equation}\label{expectation}
\begin{aligned}
E[e^{tu_i^2}]&=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^{\infty}e^{tx^2}e^{-\frac{x^2}{2}}dx=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^{\infty}e^{-\frac{x^2}{2}(1-2t)}dx\\
&=\frac{1}{\sqrt{2\pi}}\frac{1}{\sqrt{1-2t}}\int_{-\infty}^{\infty}e^{-\frac{y^2}{2}}dy=\frac{1}{\sqrt{1-2t}}
\end{aligned}
\end{equation}
where we choose $y=\sqrt{1-2t}\cdot x$ and we need $t<\frac{1}{2}$.\\
Combine Eq. \eqref{norm_bound} and Eq. \eqref{expectation}, we have
\begin{equation}\label{norm_bound2}
\begin{aligned}
P(\Vert\bm{u}\Vert^2>a^2)&\leq\frac{(1-2t)^{-\frac{d}{2}}}{e^{ta^2}}=(1-2t)^{-\frac{d}{2}}e^{-ta^2}\\
\end{aligned}
\end{equation}
Define $f(t)=(1-2t)^{-\frac{d}{2}}e^{-ta^2}$, we have:
\begin{equation*}
\begin{aligned}
f'(t)=-\frac{d}{2}(1-2t)^{-\frac{d}{2}-1}e^{-ta^2}+(1-2t)^{-\frac{d}{2}}e^{-ta^2}(-a^2)\\
\end{aligned}
\end{equation*}
Let $f'(t)=0$, we have
\begin{center}
	$$-\frac{d}{2}(1-2t)^{-\frac{d}{2}-1}(-2)e^{-ta^2}+(1-2t)^{-\frac{d}{2}}e^{-ta^2}(-a^2)=0$$
	$$d+(1-2t)(-a^2)=0$$
	$$(1-2t)=\frac{d}{a^2}$$
\end{center}
Thus, $t=\frac{1}{2}(1-\frac{d}{a^2})<\frac{1}{2}$. Using this into Eq. \eqref{norm_bound2}, we have:
\begin{equation}
\begin{aligned}
P(\Vert\bm{u}\Vert^2>a^2)&\leq(\frac{d}{a^2})^{-\frac{d}{2}}e^{-\frac{1}{2}(a^2-d)}=d^{-\frac{d}{2}}e^{\frac{d}{2}}a^de^{-\frac{a^2}{2}}
\end{aligned}
\end{equation}
For $0<\hat{\epsilon}<1$, we choose $a=c'\cdot\sqrt{\frac{d}{\hat{\epsilon}}}$ so that $t>0$ always holds. Besides, choose $c'>1$ large enough such that $P(\Vert\bm{u}\Vert^2>a^2)\leq B^{-2}a^{-8}$, we have
\begin{equation*}
\begin{aligned}
\Vert\bm{s}_i\Vert
&\leq B+Ba^2+\frac{lv}{2}a^3=B+\frac{Bc'^2d}{\hat{\epsilon}}+\frac{lvc'^3}{2}\frac{d^{1.5}}{\hat{\epsilon}^{1.5}}\\
&\leq B+\frac{Bc'^2d}{\hat{\epsilon}}+\frac{c'^2}{2\hat{\epsilon}^{0.5}}\leq\frac{3Bc'^2d}{\hat{\epsilon}}=:\mu
\end{aligned}
\end{equation*}
Combing with Eq. \eqref{p_bound}, we can say given $m$ samples of $\bm{s}_i^{'}$, with probability at least $1-mp$, $\forall i=1,...,m$. $\Vert\bm{u}_i\Vert\leq a$. In this case, based on \citep{2017arXiv170505933K} Lemma 18, we have vector Bernstein Inequality that for $0<\hat{\epsilon}<\frac{\sigma^2}{\mu}=\frac{2(d+5)}{3d}B\hat{\epsilon}$, which is always true for a $B>1.5$, we have 
\begin{equation*}
P\big(\Vert\hat{\nabla}-\nabla f_v\Vert\geq\frac{\epsilon}{2}\big)\leq \exp\big(-m\cdot\frac{\epsilon^2}{32\sigma^2}+\frac{1}{4}\big)
\end{equation*}
Choosing $m>\frac{32\sigma^2}{\hat{\epsilon}^2}(\log\frac{2}{\hat{\epsilon}}+\frac{1}{4})$, we have $P\big(\Vert\hat{\nabla}-\nabla f_v\Vert\leq\frac{\hat{\epsilon}}{2}\big)\geq 1-\frac{\hat{\epsilon}}{2}$\\
Thus, by union bound, the final probability that $\Vert\hat{\nabla}-\nabla\Vert\leq\hat{\epsilon}$ is at least
\begin{equation*}
1-mp-\frac{\hat{\epsilon}}{2}\geq 1-\frac{32{c'}^2(d+5)B^2}{\hat{\epsilon}^2}(\log\frac{1}{\hat{\epsilon}}+\frac{1}{4})\frac{\hat{\epsilon}^4}{{c'}^8d^4B^2}-\frac{\hat{\epsilon}}{2}\overset{(a)}\geq 1-(\frac{1}{4}+\frac{1}{4})\hat{\epsilon}+\frac{\hat{\epsilon}}{2}\geq 1-\hat{\epsilon}
\end{equation*}
By choose $c'\geq3$, the inequality $(a)$ holds. Thus, we finish the proof of Lemma \ref{lemma_GE}.

\begin{comment}
	For $\epsilon\geq1$, we choose $a=c\cdot\sqrt{d}\epsilon^{\frac{1}{3}}$, and $c>1$ large enough such that $P(\Vert\bm{u}\Vert^2>a^2)\leq a^{-6}$, we have
	\begin{equation}
	\begin{aligned}
	\Vert\bm{s}_i\Vert
	&\leq B+Ba^2+\frac{lv}{2}a^3=B+Bc^2d\epsilon^{\frac{2}{3}}+\frac{lvc^3}{2}d^{1.5}\epsilon\\
	&\leq B+Bc^2d\epsilon^{\frac{2}{3}}+\frac{c^2\epsilon^2}{2}\leq 3Bc^2d\epsilon^2=\mu
	\end{aligned}
	\end{equation}
	Combing with section 1, we can say given $n$ samples of $\bm{s}_i^{'}$, with probability at least $1-mp$, $\forall i=1,...,m$.\\
	In this case, choose $\sigma'^2=\sigma^2\epsilon^3>\sigma^2$, based on Jonas17, we have vector Bernstein Inequality that for $0\leq\epsilon\leq\frac{\sigma^2}{\mu}\leq\frac{\sigma'^{2}}{\mu}=\frac{2}{3}B\epsilon$, which is always true, we have 
	\begin{equation}
	P\big(\Vert\hat{\nabla}-\nabla f_v\Vert\geq\frac{\epsilon}{2}\big)\leq \exp\big(-m\cdot\frac{\epsilon^2}{32\sigma^2}+\frac{1}{4}\big)
	\end{equation}
	Choosing $m>\frac{32\sigma'^2}{\epsilon^2}(\log\epsilon+\frac{1}{4})=32\epsilon\sigma^2(\log\epsilon+\frac{1}{4})$, we have $P\big(\Vert\hat{\nabla}-\nabla f_v\Vert\leq\frac{\epsilon}{2}\big)\geq 1-\frac{1}{\epsilon}$\\
	Thus, the final probability that $\Vert\hat{\nabla}-\nabla\Vert\leq\epsilon$ is at least
	\begin{equation}
	1-mp-\frac{1}{\epsilon}\geq 1-32\epsilon\sigma^2(\log\epsilon+\frac{1}{4})\frac{1}{c^6d^3\epsilon^{2}}-\frac{1}{\epsilon}\geq 1-\frac{2}{\epsilon}
	\end{equation}	
\end{comment}
	
\end{proof}
